LeMoLE: LLM-Enhanced Mixture of Linear Experts for Time Series Forecasting

Recent research has shown that large language models (LLMs) can be effectively used for real-world time series forecasting due to their strong natural language understanding capabilities. However, aligning time series into semantic spaces of LLMs comes with high computational costs and inference complexity, particularly for long-range time series generation. Building on recent advancements in using linear models for time series, this paper introduces an LLM-enhanced mixture of linear experts for precise and efficient time series forecasting. This approach involves developing a mixture of linear experts with multiple lookback lengths and a new multimodal fusion mechanism. The use of a mixture of linear experts is efficient due to its simplicity, while the multimodal fusion mechanism adaptively combines multiple linear experts based on the learned features of the text modality from pre-trained large language models. In experiments, we rethink the need to align time series to LLMs by existing time-series large language models and further discuss their efficiency and effectiveness in time series forecasting. Our experimental results show that the proposed LeMoLE model presents lower prediction errors and higher computational efficiency than existing LLM models.

==> univariate_table/Ablation_multi_experts.tex <==
\begin{table*}[h!]
\centering
\caption{Ablations study on four datasets with different prediction lengths. A lower value indicates better performance. The best results are highlighted in bold.}
\vspace{-2mm}
\label{tab:ablation_multi_experts}
\begin{center}
\begin{small}
\scalebox{0.75}{
\setlength\tabcolsep{3pt}

\begin{tabular}{c|cc|cc|cc|cc|cc|cc|cc|cc}
\toprule
Long-term Forecasting & \multicolumn{2}{c|}{ECL-96} & \multicolumn{2}{c|}{ECL-192} & \multicolumn{2}{c|}{ECL-336} & \multicolumn{2}{c|}{ECL-720} & \multicolumn{2}{c|}{ETTh1-96} & \multicolumn{2}{c|}{ETTh1-192} & \multicolumn{2}{c|}{ETTh1-336} & \multicolumn{2}{c}{ETTh1-720} \\
\midrule
\multicolumn{1}{c|}{Metric} & MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE \\
\midrule
4 experts & 0.319 & 0.443 & 0.257 & 0.374 & 0.262 & 0.385 & 0.323 & 0.437 & 0.053 & 0.178 & 0.069 & 0.206 & 0.083 & 0.231 & 0.092 & 0.239 \\
3 experts & 0.233 & 0.339 & 0.274 & 0.403 & 0.270 & 0.396 & 0.254 & 0.379 & 0.056 & 0.183 & 0.073 & 0.211 & 0.082 & 0.229 & 0.089 & 0.236 \\
2 experts & 0.319 & 0.438 & 0.294 & 0.413 & 0.278 & 0.392 & 0.247 & 0.374 & 0.061 & 0.192 & 0.076 & 0.216 & 0.083 & 0.231 & 0.087 & 0.234 \\
1 experts & 0.310 & 0.419 & 0.241 & 0.373 & 0.299 & 0.422 & 0.284 & 0.403 & 0.062 & 0.194 & 0.075 & 0.216 & 0.084 & 0.231 & 0.086 & 0.233 \\
\midrule
\multicolumn{1}{c|}{Metric} & \multicolumn{2}{c|}{ETTm1-96} & \multicolumn{2}{c|}{ETTm1-192} & \multicolumn{2}{c|}{ETTm1-336} & \multicolumn{2}{c|}{ETTm1-720} & \multicolumn{2}{c|}{Traffic-96} & \multicolumn{2}{c|}{Traffic-192} & \multicolumn{2}{c|}{Traffic-336} & \multicolumn{2}{c}{Traffic-720} \\
\midrule
4 experts & 0.027 & 0.123 & 0.039 & 0.152 & 0.053 & 0.175 & 0.074 & 0.210 & 0.149 & 0.244 & 0.160 & 0.254 & 0.154 & 0.260 & 0.179 & 0.281 \\
3 experts & 0.027 & 0.124 & 0.041 & 0.152 & 0.054 & 0.177 & 0.074 & 0.210 & 0.163 & 0.263 & 0.148 & 0.245 & 0.147 & 0.242 & 0.168 & 0.269 \\
2 experts & 0.027 & 0.124 & 0.040 & 0.152 & 0.055 & 0.177 & 0.074 & 0.210 & 0.186 & 0.294 & 0.149 & 0.247 & 0.141 & 0.240 & 0.168 & 0.266 \\
1 experts & 0.027 & 0.126 & 0.041 & 0.155 & 0.053 & 0.175 & 0.074 & 0.208 & 0.169 & 0.268 & 0.157 & 0.258 & 0.149 & 0.250 & 0.159 & 0.261 \\
\bottomrule
\end{tabular}
}
\end{small}
\end{center}
\end{table*}

